Value as Memory: Online Value-Guided Post-training for General Robot Policies

Real-world post-training of generalist robot policies faces two challenges: partial observability makes action selection ambiguous, while offline post-training methods delay feedback from deployment experience. We present Value as Memory (VaM), a framework that addresses these challenges through value caching and online real-world reinforcement learning (RL). Value caching conditions actions on recent value predictions as task-progress memory, while online updates enable timely policy improvement by combining offline demonstrations, off-policy interventions, and on-policy rollouts for sample-efficient adaptation. As a result, VaM transitions from offline RL warmup to online autonomous learning with sparse rewards. Across long-horizon tasks involving deformable objects and contact-rich manipulation, VaM yields a mean absolute success-rate gain of $29.4\%$ with value caching, while achieving a $32.8\%$ gain with online autonomous learning over matched offline training. The evaluated online schedule performs $8\times$ as many policy iterations under the same gradient-step budget, with more than $2\times$ lower recorded time per gradient step with concurrent data collection and training.

==> exp_fig/analysis/review-evidence/outputs/checkpoint-rows.tex <==
% Generated by exp_fig/analysis/review-evidence/summarize.py
\textit{Box Assembly} & 8 & $96.25$ & $80.00$ & $16.25$ \\
\textit{Laundry Folding} & 3 & $88.89$ & $48.89$ & $40.00$ \\
\textit{Magnetic Bus Assembly} & 4 & $75.00$ & $37.50$ & $37.50$ \\


==> exp_fig/analysis/review-evidence/outputs/recovery-rows.tex <==
% Generated by exp_fig/analysis/review-evidence/summarize.py
\textit{Box Assembly} & VaM & 24/44 & 180 & $54.5$ \\
 & VaM (w/o value caching) & 35/70 & 180 & $50.0$ \\
 & VaM (w/o offline RL warmup) & 20/79 & 180 & $25.3$ \\
 & RECAP & 36/85 & 180 & $42.4$ \\
\midrule
\textit{Laundry Folding} & VaM & 38/44 & 45 & $86.4$ \\
 & VaM (w/o value caching) & 30/51 & 45 & $58.8$ \\
 & VaM (w/o offline RL warmup) & 48/66 & 45 & $72.7$ \\
 & RECAP & 49/64 & 45 & $76.6$ \\
\midrule
\textit{Magnetic Bus Assembly} & VaM & 5/15 & 40 & $33.3$ \\
 & VaM (w/o value caching) & 2/27 & 40 & $7.4$ \\
 & VaM (w/o offline RL warmup) & 9/33 & 40 & $27.3$ \\
 & RECAP & 4/30 & 40 & $13.3$ \\


==> exp_fig/analysis/review-evidence/outputs/replacement-main-rows.tex <==
% Generated by exp_fig/analysis/review-evidence/summarize.py
\review{\textbf{VaM (demo-trained value)}} & \review{$80.0\,{\color{gray}\pm 13.2}$} & \review{$71.1\,{\color{gray}\pm 20.4}$} & \review{$40.0\,{\color{gray}\pm 10.0}$} \\
\review{\textbf{VaM (post-warmup value)}} & \review{$85.0\,{\color{gray}\pm 13.2}$} & \review{$68.9\,{\color{gray}\pm 10.2}$} & \review{$50.0\,{\color{gray}\pm 10.0}$} \\


==> exp_fig/analysis/review-evidence/outputs/timing-rows.tex <==
% Generated by exp_fig/analysis/review-evidence/summarize.py
\textit{Box Assembly} & \textit{Offline RL} & $4.885\,{\color{gray}\pm 0.413}$ & 6.514 \\
 & \textit{Online RL} & $1.887\,{\color{gray}\pm 0.107}$ & 2.516 \\
\textit{Laundry Folding} & \textit{Offline RL} & $5.090\,{\color{gray}\pm 0.345}$ & 7.069 \\
 & \textit{Online RL} & $2.253\,{\color{gray}\pm 0.057}$ & 3.129 \\
\textit{Magnetic Bus Assembly} & \textit{Offline RL} & $5.891\,{\color{gray}\pm 0.105}$ & 7.213 \\
 & \textit{Online RL} & $2.571\,{\color{gray}\pm 0.160}$ & 3.061 \\

